Fast Convergence of Regularized Learning in Games

We show that natural classes of regularized learning algorithms with a form of recency bias achieve faster convergence rates to approximate efficiency and to coarse correlated equilibria in multiplayer normal form games. When each player in a game uses an algorithm from our class, their individual regret decays at $O(T^{-3/4})$, while the sum of utilities converges to an approximate optimum at $O(T^{-1})$--an improvement upon the worst case $O(T^{-1/2})$ rates. We show a black-box reduction for any algorithm in the class to achieve $\tilde{O}(T^{-1/2})$ rates against an adversary, while maintaining the faster rates against algorithms in the class. Our results extend those of [Rakhlin and Shridharan 2013] and [Daskalakis et al. 2014], who only analyzed two-player zero-sum games for specific algorithms.

==> experiment_zero_sum.tex <==
% !TEX root=fast_convergence.tex



==> polymatrix.tex <==
% !TEX root=fast_convergence.tex


\vscomment{ADD HERE PROOF that combines Daskalakis polymatrix games with our techniques to show fast convergence to equilibrium in multiplayer polymatrix games.}

==> recency_bias.tex <==
% !TEX root=fast_convergence.tex

We show that both algorithms in the previous sections can be altered to allow any finite window recency bias or with an exponentially discounted recency bias, while still leading to faster rate of convergence. We present our theorems for the optimistic FTRL algorithm, but analog results also hold for OMD. 



